Understanding Lua's Garbage Collection -- Towards a Formalized Static Analyzer

We provide the semantics of garbage collection (GC) for the Lua programming language. Of interest are the inclusion of finalizers(akin to destructors in object-oriented languages) and weak tables (a particular implementation of weak references). The model expresses several aspects relevant to GC that are not covered in Lua's documentation but that, nevertheless, affect the observable behavior of programs. Our model is mechanized and can be tested with real programs. Our long-term goal is to provide a formalized static analyzer of Lua programs to detect potential dangers. As a first step, we provide a prototype tool, LuaSafe, that typechecks programs to ensure their behavior is not affected by GC. Our model of GC is validated in practice by the experimentation with its mechanization, and in theory by proving several soundness properties.

==> conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

We give a small-step operational semantics for a large subset of the Lua
programming language, as specified both by its informal reference manual and by
its reference implementation. 

The semantics tackles the majority of the complex features of Lua, such as 
its metatable mechanism, dynamic execution of source code, error handling 
and several other standard library functions. It is defined in a modular way, 
and could be extended to tackle absent features, such as coroutines \cite{moura} 
and garbage collection \cite{ammm}, without modifying the essence of what is already 
specified. 

We provide a mechanization of the formal semantics in PLT Redex.
The portion of the test suite for the reference interpreter, which is of
interest for our model, has been successfully tested against this 
mechanization, providing evidence that we are successfully modeling the
behavior of the language. 

The development of the formal semantics, its mechanization, and its test suite
make up a tool that both semanticists and Lua developers can use for
understanding and extending the features of the language.

There are several further avenues for development: adding missing
features as coroutines, \KW{goto} statements, new operators,
large integer types of version 5.3 and garbage collector. Among them,
the \KW{goto} statement would require using a slightly different
notion of a concept already in use in our model: evaluation contexts
that maintain the portions of the program already
executed, as used in \cite{seplogic}. The small step style of the semantics
of our model seems to be adequate for modeling non-local control and 
the interaction between goto statements and block-scoped variables, as 
argued in the cited work. It remains as a future work to cope with the
remaining complexities of the semantics of the statement.

The formal semantics and its mechanization can provide a basis for specifying, 
implementing, and formally proving correct static analyses for Lua programs.
There are already some tools and language extensions that do this\footnote{Such as 
Luacheck (\url{https://github.com/mpeterv/luacheck}), Ravi (\url{http://ravilang.github.io}), 
and Typed Lua~\cite{typedlua}.}, but they currently have no formal guarantee of 
correctness.

In proving desired properties of the model (fundamentally, progress property), we
choose to let as a future work the developing of a tool for assisting in the translation 
of our PLT Redex model to a Coq model. In that way, we can offer a mechanization
ready to use by a broader audience, while also having a quick escape to a proof assistant, 
to verify properties of each iteration of the PLT Redex model.

% The first avenue is
% coverage of coroutines, the biggest missing feature in our formalization.
% There is a reduction semantics for Lua-style coroutines~\cite{moura}
% that could be adapted for this purpose. 

% Another avenue is updating the semantics to the current version of 
% the language, Lua 5.3, which added 64-bit integers as a second numeric
% type, new bitwise operators (with associated fallbacks in the metatable
% mechanism) for them, and several changes in the standard library that
% altogether break compatibility with the previous language. 

% A third avenue is modelling the C API, the foreign function interface that Lua 
% uses both for interaction with a host program and interaction with native 
% libraries (including the implementation of the standard library in the 
% reference interpreter). Unlike the foreign function interfaces of
% other scripting languages, Lua's C API is uncoupled from implementation
% details of its interpreter~\cite{needle}.

% Finally, the formal semantics and its mechanization can provide a
% basis for specifying, implementing, and formally proving correct
% static analyses for Lua programs. There are already some tools and language 
% extensions that do this\footnote{Such as Luacheck (available at https://github.com/mpeterv/luacheck), Ravi (available at http://ravilang.github.io), 
% and Typed Lua~\cite{typedlua}.},
% but they currently have no formal guarantee of correctness.

%  LocalWords:  Luacheck Ravi


==> mechanization.tex <==
\section{Mechanization}
\label{sec:mechanization}


\begin{figure}
\begin{tabular}{|c|c|c|} \hline
\textbf{File}    & \textbf{Features tested}& \textbf{Coverage}\\ \hline
calls.lua        & functions and calls     & 77.83\%\\ \hline
closure.lua      & closures                & 48.5\%\\ \hline
constructs.lua   & syntax and              & 63.18\%\\ 
                 & short-circuit opts.     &        \\ \hline
events.lua       & metatables              & 90.4\%\\ \hline
locals.lua       & local variables         & 62.3\%\\ 
                 & and environments        &      \\ \hline
math.lua         & numbers and             & 82.2\%\\ 
                 & math lib                &       \\ \hline
nextvar.lua      & tables, next, and for   & 53.24\%\\ \hline
sort.lua         & (parts of) table        & 24.1\%\\ 
                 & library                 & \\ \hline
%strings.lua      & strings and string      & ?\\ 
%                 & library                 & \\ \hline
vararg.lua       & vararg                  & 100\%  \\ \hline
\end{tabular}
\caption{Lua 5.2's test suite coverage.}
\flabel{test_suite}
\end{figure}

The formalization of the semantics was carried in parallel with its
mechanization in PLT Redex~\cite{plt}.  This tool helped us recognize
problems in our first attempts at formalizing Lua, and allowed us to experiment
with new ideas before adding them to the formalization. It also allowed us to
execute part of test suite of the reference interpreter of the language\footnote{Available at https://www.lua.org/tests/.},
providing evidence that our semantics is in compliance with it.

We could not use the whole test suite, for the following reasons:
\begin{compactitem}
\item Language features not covered by our formalization: coroutines, the 
\KW{goto} statement, garbage collection, some standard library functions 
(mostly related with file handling) and other standard libraries implemented in
C (\textsf{bit32}, \textsf{coroutine}, \textsf{debug}, \textsf{io}, etc).
\item Several other tests for implementation details of the
interpreter, and not the language. According to the Lua authors, the
goal of the test suite is to test their reference {\em implementation} of Lua,
and not to serve as a conformance test for alternative implementations\footnote{
https://www.lua.org/wshop15/Ierusalimschy.pdf}.
\end{compactitem}

In practice, from the 25 \textsf{.lua} files present in the test suite,
which actually test some feature of the language, we are
able to port and run 9 against our PLT Redex mechanization. \fref{test_suite}
shows the percentage of LOCs actually tested from each of these remaining files, totaling
1256 LOCs successfully tested. Each file from the test suite is a
sequence of assertions about the expected outcome of valid code as well as code 
that generates errors.
It is important to remark that every file and line not tested is for the reasons
explained above, and every line (in the 9 files tested) that fall within the scope
of this work successfully passes the test. We take this as strong evidence that
the mechanization of our formal semantics behaves exactly the same as the
reference Lua interpreter.

Unfortunately, we do not have the space to discuss the code, which we plan to do
in an extended version of this article. For the moment, we refer the reader to
the documentation accompanying the code attached as supplementary material.

% We must note that the mechanization provided not only plays the role of a
% tool with which we can obtain evidence of conformity between our model and
% the actual implementation of Lua. It also can be used for rapid prototyping
% of new features for the language. Explore this application of the mechanization
% would require a whole article devoted to it. For reasons of space,
% we refer the reader to the documentation accompanying the mechanization
% provided.
% With respect to the testing of errors, via the module \textsf{errors.lua},
% we left it out because its implementation is heavily based on
% the services \textsf{string.find}, \textsf{string.gsub} and 
% \textsf{string.format}, which are not included in our model (though the
% principal difficulty in their implementation resides on compiling Lua's
% pattern matching expression to Racket's one).

\paragraph*{Dynamic loading of code}
By implementing our parser directly in Racket (the language upon which
PLT Redex is based), we mechanized easily the \textsf{load}
service: Lua's compiler available at runtime. 

% The mechanization made
% successfully passed every use case of the \textsf{load} service
% found on the portion of test suite pertinent to our model.

There are several details to mention related to the solution implemented,
but for reasons of space we point out the most prominent:
\begin{itemize}
\item It covers the two modes: when the program to be compiled is passed as a
  string, or when it is a function from which the service obtains the program's
  string.
    
    \item It can handle the compilation of code on a modified
    global environment.
    
    \item For completion, we emulate the case of the compilation of
    \textit{binary chunks} (that is, a pre-compiled version of
    the code). This feature is implemented in conjunction with
    the service \textsf{string.dump}, which returns
    a string containing a binary representation
    of a function, given as a parameter.
 % The details of 
 %    representation are of no interest. Which is indeed important
 %    is the relation that should hold between \textsf{load} and \textsf{string.dump}.
 %    We haven been able to test our solution over test cases
 %    found in the Lua 5.2' test suite.
  \end{itemize}

  \subsection{Garbage collection}
  The declarative nature of the given formalization of GC makes it unsuitable
  for its mechanization with Redex. \todo{Completar}

  To that end, we need a primitive recursive definition or at least a
  well-founded one. We propose the following:

  \begin{quote}
  \small
  \begin{tabbing}
    $\mathsf{stReachGCTE(\Var{e}_1, \Var{t}, \sigma, \theta_1)}$ = \= 
    $\mathsf{\Var{e}_1 \in \Var{t} \; \vee}$\\
    \> $\mathsf{[\exists \; \Var{o} \in \Var{t},}$ \= 
    $\mathsf{(\Var{k}, \Var{v}) \in SO(\Var{o}, \theta_1),}$\\
    \>\> $\mathsf{[\Var{k} \notin \Var{gcte} \; \vee \;
      stReachGCTE(\Var{k}, \Var{t}, \sigma, \theta_2)] \; \wedge}$\\
    \>\> $\mathsf{stReachGCTE(\Var{e}_1, \Var{v}, \sigma, \theta_2)] \; \vee}$\\
    \> $\mathsf{[\exists \; \Var{o} \in \Var{t},}$ \= 
    $\mathsf{\Var{v} \in SO(\Var{o}, \theta_1),}$\\
    \>\>$\mathsf{stReachGCTE(\Var{e}_1, \Var{v}, \sigma, \theta_3)] \; \vee}$\\
    \> $\mathsf{\exists \; \Var{r} \in \Var{t}, \; 
      stReachGCTE(\Var{e}_1, \sigma(\Var{r}), \sigma \backslash \{ \Var{r} \},
      \theta_1)}$\\\\
    
    $\mathit{where} \; \mathsf{\theta_2 = \theta_1[\Var{o} := 
        \theta_1(\Var{o})[1 := \theta_1(\Var{o})(1) \backslash \{ \Var{k} \}] \; ]}$\\\\

   $\mathsf{\theta_3 =}
        \left\{
        \begin{array}{lcl}
          \mathsf{
          \theta_1[\Var{o} := 
          \theta_1(\Var{o})[1 := \theta_1(\Var{o})(1) \backslash \{ \Var{v} \} ] \;
          \mathit{if} \; wv?(\Var{o}, \theta) \; \wedge \; \neg wk?(\Var{o}, \theta)}\\

          % \mathsf{
          % \left.\theta_1\right|_{dom(\theta_1) - \{ \Var{o} \}} \cup 
          % \{ \Var{o} \rightarrow 
          % \theta_1(\Var{o})[1 :=
          % \left.\theta_1(\Var{o})(1)\right|_{dom(\theta_1(\Var{o})(1)) - \{ \Var{v}_2 \}}] \} \;
          % \mathit{if} \; \neg wv?(\Var{o}, \theta) \; \wedge \;
          % \neg wk?(\Var{o}, \theta) \; \Var{v}_2 \in dom(\theta_1(\Var{o})(1))}\\

          \mathsf{
          \theta_1[\Var{o} := \theta_1(\Var{o})[1 := 
          (\left.\bigcup\limits_{
          \substack{\Var{k} \; \in \; dom(\Var{t})\\ 
          \Var{t}(\Var{k}) \; = \; \Var{v}}} t[\Var{k} := \nil])
          \right|_{
          \substack{\mathsf{\Var{k} \; \in \; dom(t)} \\ 
          \mathsf{\Var{k} \neq \Var{v}}}} \cup
          \bigcup\limits_{
          \substack{\Var{k} \; \in \; dom(\Var{t})\\
          \Var{k} \; = \; \Var{v}}} 
          \{ (\Var{t}(\Var{k}), \Var{t}(\Var{k})) \} \;
          \mathit{o/w}}
        \end{array}
        \right.$ 
  \end{tabbing}     
\end{quote}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:

%  LocalWords:  lua nextvar vararg coroutine io

